Towards Observability for Production Machine Learning Pipelines

Software organizations are increasingly incorporating machine learning (ML) into their product offerings, driving a need for new data management tools. Many of these tools facilitate the initial development of ML applications, but sustaining these applications post-deployment is difficult due to lack of real-time feedback (i.e., labels) for predictions and silent failures that could occur at any component of the ML pipeline (e.g., data distribution shift or anomalous features). We propose a new type of data management system that offers end-to-end observability, or visibility into complex system behavior, for deployed ML pipelines through assisted (1) detection, (2) diagnosis, and (3) reaction to ML-related bugs. We describe new research challenges and suggest preliminary solution ideas in all three aspects. Finally, we introduce an example architecture for a "bolt-on" ML observability system, or one that wraps around existing tools in the stack.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> coarse-grained-Jul-11-surgery-bkp.tex <==
%!TEX root = main.tex
\newpage

\subsection{Detecting ML Performance Issues}
\label{sec:coarsegrained}

% \rtwo{Post-deployment, the starting point for identifying issues
% is estimating real-time performance using metrics such as accuracy. 
% However, even a simple estimate of accuracy becomes challenging when labels 
% on predictions are delayed or absent. 
% Moreover, delays may not be uniform across
% buckets
% (e.g., a power outage in East Village 
% might prevent taxicab meter information 
% from being uploaded) and 
% can be exacerbated in situations where 
% manual labeling is required. 
% As shown in Figure~\ref{fig:tradpipeline}, 
% predictions and feedback arrive 
% at different timestamps and 
% are joined on some identifier. 
% At every timestamp, ML pipelines can move 
% between three feedback scenarios: 
% no feedback, partial feedback, and full feedback. 
% The challenges stem from two issues:
% first, the lack of labels (which impacts the partial and no feedback settings)
% and 
% We start by discussing 
% We discuss each of the feedback scenarios in turn.}



\rtwo{There are a handful of detection challenges, such as large-scale joins of prediction and feedback (i.e., labels), efficiently tracking custom distance metrics between current and historical model score distributions, and computing pipeline metrics with low latency, that can be solved with straightforward adaptations of prior work \shreya{TODO: cite}. However, a major pain point faced almost universally ---  many false positive ML performance drop alerts --- is unaddressed. We propose approximating top-line ML metrics (e.g., accuracy) and monitoring changes in real-time; the biggest challenge here is that labels on predictions 
can be delayed. \shreya{TODO: cite} Moreover, delays may not be uniform across 
different buckets 
(e.g., a power outage in East Village 
might prevent taxicab meter information 
from being uploaded) and 
can be exacerbated in situations where 
manual labeling is required. 
As shown in Figure~\ref{fig:tradpipeline}, 
predictions and feedback arrive 
at different timestamps and 
are joined on some identifier. 
At every timestamp, ML pipelines can move 
between three feedback scenarios: 
no feedback, partial feedback, and full feedback, impacting real-time accuracy scores. We discuss each of the feedback scenarios in turn.}



\subsubsection{No-Feedback}
\label{sec:nofeedback}

This scenario typically occurs 
immediately after deployment. 
% Suppose we have two sources of raw data: 
% taxi sensor telemetry data (e.g., mileage, location) 
% to generate predictions from and meter data 
% (e.g. payment information) as feedback. 
% \agp{Why is this introduced here? Maybe want to move this up?} \shreya{I don't think we even need the sentence, so I deleted it.}
The feedback might come in batches at a later date, 
possibly after human review, motivating us to 
find ways to estimate real-time performance without labels.  

To estimate cumulative accuracy, 
we may use importance weighting 
(IW) techniques~\cite{sugiyama}. 
At a high level, we can identify buckets 
based on input features or combinations thereof, 
determine the training set accuracy 
for each bucket, and weight these accuracies 
based on the number of points in each bucket 
in the live (post-deployment, unlabeled) data. 
Consider the neighborhood 
as a naive bucketing strategy: if the 
training set had FiDi and Midtown accuracies 
of 80\% and 50\% respectively and we have 
100 FiDi and 500 Midtown live predictions, 
we can estimate an accuracy of $0.8 \times 100 + 0.5 \times 500 = 55\%$. 


\begin{figure}
\vspace{-8pt}
    \centering
    \includegraphics[width=\linewidth]{figs/bucketings.pdf}
    \vspace{-15pt}
    \caption{Bucketing strategies based on pickup location and trip distance. 1-D histograms are normalized to show density. As buckets become more finer-grained, they also become sparse.}
    \label{fig:bucketings}
    \vspace{-15pt}
\end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figs/feb1.pdf}
%         \caption{Difference between pickup locations in month of January 2020 and the week of February 1, 2020.}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{figs/mar28.pdf}
%         \caption{Difference between pickup locations in month of January 2020 and the week of April 18, 2020.}
%     \end{subfigure}
%     \caption{Example of bucketing strategy based on pickup location. The distributions may diverge more as time goes on, potentially impacting the correctness of the accuracy estimate in the no-feedback case.}
%      \label{fig:locationhists}
% \end{figure}


An open question here is which bucketing strategy to use.
Even if we decide to construct the bucketing offline\techreport{ and not
change it in response to live data}, there are still
many candidate bucketings.
We can construct bucketings based on any subset of the input features,
which is $O(n!)$, where $n$ is the number of features.
Figure~\ref{fig:bucketings} illustrates three bucketings. 
The first couple of bucketings have representation 
in each bucket, which gives us some confidence in per-bucket accuracy. 
However, the last bucketing has some buckets 
with zero representation---so if a live tuple were to be assigned to such a bucket, we would not have an accuracy estimate for it.
Overall, finer-grained bucketings may capture
patterns not found in coarse-grained bucketings
but could also 
be more sparse, which can impact the 
correctness of our accuracy estimates.
The goal overall is to produce the closest 
approximation of accuracy\techreport{ (or any chosen coarse-grained metric)},
while bounding the number of buckets\techreport{ (a proxy for storage)}. 
Therefore, a "good" bucketing strategy 
must have lots of diversity among different buckets
but little diversity within individual buckets---analogous
to typical clustering objectives. \rtwo{Furthermore, while in Figure~\ref{fig:bucketings}, location is a simple bucketing strategy and thus explainable; more complicated bucketing strategies may be less interpretable for users.}
Additionally, each bucket 
should have substantial representation in the 
training set: if the number of training tuples 
for a bucket is small, we cannot be confident in the live IW estimate.
Picking the bucketing 
is also related to statified sampling~\cite{parsons2014stratified},
used in AQP~\cite{agarwal2013blinkdb,acharya1999aqua}
to support predicates on the stratified attributes.
Inspired by recent "hybrid AQP" work,  
we can also construct different bucketings 
and merge the resulting accuracy estimates~\cite{sanjayaggaqp}.

\strikeout{Extending this technique to the sliding window accuracy setting if
we are using a fixed offline bucketing may be straightforward.
Per bucket, we can apply ideas from prior work 
in streaming algorithms to update 
counts for the last $n$ tuples~\cite{datar2002maintaining}; 
similar techniques may also apply for the sliding window defined by time.}


Finally, we may gain additional benefits from changing
the bucketing strategy in response to live data. 
The research challenge is then to devise methods that 
efficiently identify buckets in high-dimensional, 
changing data streams with a reference dataset 
in mind (i.e., the training set). 
A starting point to a solution could 
be to extend streaming clustering algorithms 
that are explicitly robust to changing 
data distributions~\cite{Mousavi2015DataSC}: 
in addition to the live data, 
we could feed the training set to such a clustering algorithm.


\subsubsection{Full-Feedback and Partial-Feedback}
\label{sec:partialfeedback}
\mr{In the full-feedback setting, 
we have labels or feedback 
for all the predictions so far. We can simply perform a join and compute the metric over the result; challenges only occur at scale when windows are too large to fit both predictions
and feedback in-memory, motivating AQP (approximate query processing) techniques. For example, we could maintain both a
reservoir (for prediction tuples whose
feedback has not been received) 
as well as partial aggregates (for prediction tuples whose
feedback has been received).}

\mr{Realistically, many ML pipelines will be in the partial-feedback setting: often, live data is only partially labeled or arrives 
on a specific schedule. Or, some upstream 
data collection issues might 
delay feedback (e.g., there’s 
a cell tower outage in a region of Tribeca, 
causing payment meter data to be delayed). 
Here, aggregating the full-feedback 
and no-feedback estimates, weighted by the count of tuples in each case, 
may produce a reasonable real-time accuracy estimate.}
% However, if feedback fails to arrive
% for certain subsets of data
% for extended periods of time, users may want to diagnose
% this matter further, as discussed in the next section.


% For a naive solution to the delayed label pattern mining challenge, we can draw inspiration from streaming pattern mining algorithms such as frequent itemsets~\cite{streamingfreqitemset}. However, such algorithms look through groups of features in windows of tuples with labels that don’t change, while the tuples we want to apply the frequent itemsets algorithm to---the ones that don’t have feedback (i.e., the “delayed” points)---might receive feedback after we compute the frequent itemsets. Consequently, how do we extend streaming frequent itemset algorithms to efficiently recompute itemsets after removing tuples? We can build on work in incremental maintenance of frequent itemsets~\cite{incmaintfreq}. \shreya{TODO: ask aditya how to reword to make sense}


\subsubsection{Full-Feedback}
\strikeout{When estimating real-time accuracy
for these predictions, 
there are at least three variants of interest:
(a) cumulative accuracy for all predictions
made until now;
(b) accuracy for predictions made in
the last time window $t$;
(c) accuracy for the last $k$ predictions.
The last two variants provide accuracies over a sliding window.
The cumulative setting is not just relevant 
when we are evaluating accuracy from $t=0$;
it is also useful when we 
reset the clock regularly, 
e.g., accuracy
on a per-day basis.}

\strikeout{To estimate 
cumulative accuracy (a)
we simply need to perform an approximate join between
the prediction and feedback streams.
Challenges occur at scale, when our streaming
windows too large to fit both predictions
and feedback in-memory, motivating AQP (approximate query processing) techniques.
A naive solution is to uniformly subsample the prediction and feedback streams before joining them to compute accuracy, but it is well-known that uniformly subsampling streams before a join can yield quadratically fewer tuples in the result~\cite{chaudhuri}. 
Unlike the standard join setting, here, each prediction tuple
joins precisely with a single feedback tuple, 
meaning that the challenges of 
quadratically fewer samples 
with AQP over joins do not 
apply~\cite{chaudhuri,kandula, joinstheoreticalguide}---however, 
new challenges emerge.
Since we do not know the size of the stream in advance, 
a naive approach is to apply
reservoir sampling~\cite{aggarwal2006biased} on both streams
using a shared hash function on the common identifier.
However, this approach is wasteful, since
once the pair of prediction and feedback tuples are received,
they no longer both need to be stored in memory.  
Moreover, the quality of the estimate degrades over time 
since we are maintaining a fixed size sample
over streams that grow in size.
Ideally we would want to maintain both a
reservoir (for prediction tuples whose
feedback has not been received) 
as well as partial aggregates (for prediction tuples whose
feedback has been received).
Joined tuples can make way for new slots in the reservoir. 
However, doing so while respecting 
the typical reservoir sampling guarantee
of each  having the same probability of being
sampled, is non-trivial.
For example, the sudden arrival of
a number of feedback tuples
can cause multiple slots in the reservoir to become
vacant, leading to an increasing probability for
the next prediction tuple to be included in the reservoir.}

\strikeout{Extending this reservoir sampling 
approach to (b) and (c) is also challenging. 
We can leverage prior work on 
reservoir sampling over 
windows~\cite{babcock2001sampling,aggarwal2006biased,gemulla2008sampling,bailis2017macrobase},
where we can evict old tuples from the reservoir
when they expire~\cite{babcock2001sampling}, or update the probabilities to
favor newer tuples more, using
an exponential decay weighting~\cite{bailis2017macrobase}. 
As before, we will want to modify these techniques to be less 
wasteful of memory, while also ensuring that they are unbiased.}

\subsubsection{Full-Feedback and Partial-Feedback}
\label{sec:partialfeedback}
\mr{In the full-feedback setting, 
we have labels or feedback 
for all the predictions so far. We can simply perform a join and compute the metric over the result; challenges only occur at scale when windows are too large to fit both predictions
and feedback in-memory, motivating AQP (approximate query processing) techniques. For example, we could maintain both a
reservoir (for prediction tuples whose
feedback has not been received) 
as well as partial aggregates (for prediction tuples whose
feedback has been received).}

\mr{Realistically, many ML pipelines will be in the partial-feedback setting: often, live data is only partially labeled or arrives 
on a specific schedule. Or, some upstream 
data collection issues might 
delay feedback (e.g., there’s 
a cell tower outage in a region of Tribeca, 
causing payment meter data to be delayed). 
Here, aggregating the full-feedback 
and no-feedback estimates, weighted by the count of tuples in each case, 
may produce a reasonable real-time accuracy estimate.}
% However, if feedback fails to arrive
% for certain subsets of data
% for extended periods of time, users may want to diagnose
% this matter further, as discussed in the next section.


% For a naive solution to the delayed label pattern mining challenge, we can draw inspiration from streaming pattern mining algorithms such as frequent itemsets~\cite{streamingfreqitemset}. However, such algorithms look through groups of features in windows of tuples with labels that don’t change, while the tuples we want to apply the frequent itemsets algorithm to---the ones that don’t have feedback (i.e., the “delayed” points)---might receive feedback after we compute the frequent itemsets. Consequently, how do we extend streaming frequent itemset algorithms to efficiently recompute itemsets after removing tuples? We can build on work in incremental maintenance of frequent itemsets~\cite{incmaintfreq}. \shreya{TODO: ask aditya how to reword to make sense}


==> component.tex <==
\begin{Verbatim}[commandchars=\\\{\},numbers=left,firstnumber=1,stepnumber=1]
\colorbox{white}{\parbox{\linewidth}{\PY{k+kn}{from} \PY{n+nn}{mltrace} \PY{k+kn}{import} \PY{n}{Component}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{\PY{k}{class} \PY{n+nc}{PreprocessingComponent}\PY{p}{(}\PY{n}{Component}\PY{p}{)}\PY{p}{:}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{k}{def} \PY{n+nf}{beforeRun}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{,} \PY{n}{df}\PY{p}{,} \PY{n}{features}\PY{p}{,} \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{n}{null\PYZus{}threshold} \PY{o}{=} \PY{l+m+mf}{0.1}\PY{p}{)}\PY{p}{:}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{n}{null\PYZus{}fracs} \PY{o}{=} \PY{n}{df}\PY{o}{.}\PY{n}{isna}\PY{p}{(}\PY{p}{)}\PY{o}{.}\PY{n}{sum}\PY{p}{(}\PY{p}{)} \PYZbs{}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{            \PY{o}{/} \PY{n}{df}\PY{o}{.}\PY{n}{shape}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{k}{if} \PY{n}{null\PYZus{}fracs}\PY{o}{.}\PY{n}{any}\PY{p}{(}\PY{p}{)} \PY{o}{\PYZgt{}} \PYZbs{}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{            \PY{n}{null\PYZus{}threshold}\PY{p}{:}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{            \PY{k}{assert} \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{Too many nulls!}\PY{l+s+s2}{\PYZdq{}}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{k}{def} \PY{n+nf}{afterRun}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{,} \PY{n}{train\PYZus{}df}\PY{p}{,} \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{n}{stdev\PYZus{}cutoff} \PY{o}{=} \PY{l+m+mf}{5.0}\PY{p}{)}\PY{p}{:}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{n}{z\PYZus{}scores} \PY{o}{=} \PY{p}{(}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{            \PY{p}{(}\PY{n}{train\PYZus{}df} \PY{o}{\PYZhy{}} \PY{n}{train\PYZus{}df}\PY{o}{.}\PY{n}{mean}\PY{p}{(} \PYZbs{} \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{                \PY{n}{axis}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{,} \PY{n}{skipna}\PY{o}{=}\PY{k+kc}{True}\PY{p}{)}\PY{p}{)} \PY{o}{/} \PYZbs{} \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{                \PY{n}{train\PYZus{}df}\PY{o}{.}\PY{n}{std}\PY{p}{(}\PY{n}{axis}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{,} \PYZbs{} \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{                \PY{n}{skipna}\PY{o}{=}\PY{k+kc}{True}\PY{p}{)}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{p}{)}\PY{o}{.}\PY{n}{abs}\PY{p}{(}\PY{p}{)}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{k}{if} \PY{p}{(}\PY{n}{z\PYZus{}scores} \PY{o}{\PYZgt{}} \PY{n}{stdev\PYZus{}cutoff}\PY{p}{)} \PYZbs{} \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{            \PY{o}{.}\PY{n}{sum}\PY{p}{(}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{l+m+mi}{0}\PY{p}{:}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{            \PY{k}{assert} \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{There are outliers!}\PY{l+s+s2}{\PYZdq{}}\vphantom{fg}}}
\end{Verbatim}

==> fine-grained-Jul-11-surgery.tex <==




\subsection{Diagnosing ML Performance Issues}
\label{sec:finegrained}

\agp{Mention refs: All three prongs are currently pain points for practitioners and require a lot of manual investigation, motivating opportunities for automation~\cite{metaobstalk, lyftarticle}. Circuitous and unmanageable ways of detecting bugs due to a lack of ground-truth labels yield false positives (as discussed in Section~\ref{sec:distshiftformal})}

 \rtwo{After detecting an ML performance drop, the next need is to diagnose it, or identify the most likely root causes. We focus on bugs that arise \emph{after} a pipeline has been deployed to production (i.e., relate to a mismatch between training and serving). In this section, we formalize a spectrum of ML errors, discuss shortcomings of existing strategies, and outline two new research challenges: learning constraints for columns and tracking slow distribution shift.}
 
\subsubsection{"Catch Me If You Can" Nature of ML Bugs}
\mr{Finding where ML bugs lie is like finding a needle in a haystack. ML errors can originate from any component in the pipeline and span the following hierarchy, from most to least time-sensitive: hard $\rightarrow$ soft $\rightarrow$ drift. Hard errors, such as some data sources failing to ingest and resulting in missing feature values, need immediate attention. Soft errors, such as a handful of features having anomalous means, require more tedious manual investigation because of the false positive problem: many columns can deviate significantly while only a few are responsible for pipeline performance drops. Finally, bugs can result from natural data drift. These bugs cause model performance to slowly decrease and thus are the least time-sensitive; nevertheless, they require attention and can be the hardest to track. \shreya{TODO: cite}}
 
 \subsubsection{Failure Modes in Existing Post-Deployment Diagnosis Strategies}
 \label{sec:provenance}
  \mr{A prerequisite for diagnosis is tracking provenance for predictions, especially in pipelines where input and output data are continuously updating~\cite{provdb} \shreya{TODO: cite more provenance literature}. Provenance is hard to get in a “bolt-on” approach, or one that does not require practitioners to rewrite their entire pipeline in a custom framework; thus, they typically diagnose at the model feature and prediction level and use "tribal knowledge" to trace misbehaving features to potential upstream causes}. 
  
\mr{Practitioners usually instrument their code with data validation and constraint checks~\cite{dataval, mlinspect, schelter, dde,dboost}.
For example, 25 different types of ML-specific data constraints on 
a single column basis, and two constraints
on pairs of columns, are defined in Schelter et al.~\cite{schelter} and often require enumerating threshold values specific to the column(s)~\cite{schelter}. While data validation is not new, the challenge lies in actually using it. Too many constraints yield false positives (i.e., a pipeline component is flagged even if downstream predictions are correct), and it can be tedious to manually define constraints for every column. As a step towards automation, TFX suggests basic hard constraints such as type checks and set membership for categorical columns. Although these can have high precision, they typically have low recall and thus are inadequate on their own~\cite{tfx}, motivating the need for soft constraints.}
  
%   To get traces for each prediction, we propose a simple solution of asking users to annotate components of a pipeline (e.g., with decorators for Python) with pointers to inputs and outputs (e.g., dataframe variables) that we automatically log to an observability store. When users want to retrieve a trace, we can compute a depth-first-search through logs on the fly. Another option is to instrument the AST or bytecode to automatically capture lineage~\cite{mlinspect}, but this forces users to remain in a particular language or framework}.



\subsubsection{Learning Soft Data Integrity Constraints on Provenance Snapshots}
\label{sec:dataconstraints}

\rtwo{Since bugs can originate from any component in the pipeline, our first challenge is to get provenance for each prediction in a bolt-on observability system. To get traces for each prediction, we propose a simple solution of asking users to annotate components of a pipeline (e.g., with decorators for Python) with pointers to inputs and outputs (e.g., dataframe variables) that automatically get logged to an observability store. When users want to retrieve a trace, we can compute a depth-first-search through logs on the fly. Another option is to instrument the AST or bytecode to automatically capture lineage~\cite{mlinspect}, but this forces users to remain in a particular language or framework.}

\rtwo{Given provenance snapshots, we can execute constraint checks on intermediate inputs and outputs and log the results; when ML performance drops are flagged, users can then trace a prediction and inspect such results to determine which component(s) to address. The key question is, what constraint checks do we execute? To take the burden of enumerating potentially thousands of constraints off the practitioner, we propose auto-generating suites of input and output validation constraints. The learned constraints should flag anomalous tuples with high precision and high recall. Ideally, the constraints are \emph{explainable} and thus more actionable, rather than float-valued column bounds that may seem random. If we have access to the user's model, we can narrow the search space by restricting constraints to columns involved in important features~\cite{Franois2006ThePT}; however, it is unrealistic to assume such access, especially for a bolt-on observability system.}

\rtwo{A solution idea is to learn an autoregressive model that predicts the likelihood of a column's value for a tuple given values of the other columns; then we can aggregate likelihood scores for each column over sliding windows of tuples. Deep autoregressive models have demonstrated success in capturing rich multivariate distributions in challenging tasks, such as cardinality estimation~\cite{cardestimation}. Leveraging conditional density estimation, a naive approach for our task is to fit an autoregressive function for each feature to model its distribution at time $t$ given the joint distribution of other features at time $t$, as well as tuples corresponding to times $< t$. However, this does not scale to more than a handful of features, so we can use masking techniques to train a single model for all features~\cite{made, bert, cardestimation}. Another challenge is that most off-the-shelf autoregressive models are trained explicitly to predict the next value or token, which will not work in our case because we need to learn the \emph{distributions} or density functions of features. Thus, we need to discretize inputs and outputs so the model learns a distribution of buckets. A simple bucketization strategy can be derived from the CDF (e.g., quantiles), but this will fail as distributions change over time. Alternatively, recent progress in language modeling suggests a different bucketization strategy --- numbers can be discretized into digits~\cite{Wallace2019DoNM}.}


\rtwo{To turn the conditional density estimation model(s) into a suite of constraints, users can define a common threshold for columns --- for example, tuples should have an aggregated column likelihood score above 80\%. We can also fine-tune the threshold based on the size of the data (i.e., number of columns and tuples) to find a good trade-off between precision and recall of alerts. Further challenges include efficiently maintaining these autoregressive models and their data (e.g., fine-tuning, running across provenance snapshots).}

% \rtwo{While the data integrity constraints provide valuable guardrails to practitioners, two other challenges remain unaddressed. First, users may want suggestions for constraints to add, both to surface checks that they may have missed and to adapt to the changing nature of data. We can use anomalies flagged by data validation to indicate new constraints. Second, which the remainder of this section will focus on, is that data might drift over time, passing data integrity constraints.}

\strikeout{However, there are two issues.
First, even with these constraints, in many cases
users simply want to go and inspect the actual raw inputs and outputs
across components in the ML pipeline.
Second, checking so many constraints
when there are thousands of features
can be quite expensive.
We consider each issue in turn.

Logging raw inputs and outputs for each component in the ML pipeline
can quickly get expensive.
As an anecdote, the first author worked at a startup where 
the MLFlow~\cite{mlflow} logs would require a "purge" every few months.
To minimize log size, 
we can use the same approach as in the previous section and use
a reservoir sample for prediction tuples; a uniform sample may suffice for 
training tuples.
In addition, we can log histograms instead of full data streams; however, bins should change as data evolves over time. Research challenges lie in combining ideas from incrementally-maintained approximate histograms with ideas from adaptive histograms to produce evolving summaries of windows of data~\cite{fastincmaint}. 
Another insight is that users will only selectively query logged intermediates (e.g., inspect the head of a dataframe). For each component, we can learn from query patterns over time to inform what goes into logs, thereby reducing latency and storage footprints. 

When checking constraints, we may want to learn how to sequence
the checking of constraints to reduce overall cost and quickly identify errors.
This problem is reminiscent of work on adaptive query processing~\cite{avnur2000eddies,babu2004adaptive} by reordering predicates
based on selectivity. We will need to adapt these techniques
for the defined space of constraints---in our case, we may be able to identify
the optimal constraint checking strategy offline. }





\subsubsection{Learning Longer-Term Distribution Shift} 
\label{sec:distshift}

Data integrity checks do not flag slower, longer-term distribution shift, 
motivating the need to track how data distributions 
change over time. For instance, a recession could cause riders to tip less across the population, changing $P(Y)$ but not $P(X)$. To approximately compute shifts in $P(X)$ and $P(Y)$, existing work proposes tracking metrics like KL divergence and KS tests~\cite{failingloudly} between sliding windows in live inference data and train datasets (i.e., for train-serve skew as described in Breck et al.~\cite{dataval}). There are two problems with this approach: (1) it requires the inference and training data to be kept in memory, and (2) it doesn't work well in settings where there are many tuples---$p$-values go to zero even if shifts aren't significant enough to warrant a retrain, as discussed in Section~\ref{sec:distshiftformal} and shown in Figure~\ref{fig:pvalues}.

\begin{figure}
\vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{figs/ks_pvalue.pdf}
    \vspace{-17pt}
    \caption{K-S test $p$-values for each feature and prediction. The training set (Jan 2020) is compared to week-long sliding windows of inference data (Feb 2020--). $p$-values are "significant" ($<0.05$) throughout. The ML model accuracy is depicted by the dashed line.}
    \label{fig:pvalues}
\vspace{-10pt}
\end{figure}

To solve (1), the memory issue, we can leverage a reservoir of live tuples (as in Section~\ref{sec:coarsegrained}), but it is impractical to keep the entire training set in memory. We can keep a materialized sample of the training set in-memory, but randomly sampling the training set might neglect important tuples, such as those from minority classes. As a solution, we can obtain a weighted random sample of the train set, where each tuple is weighted by its loss.

To solve (2), the $p$-value issue, we can draw inspiration 
from adversarial validation, a\techreport{ Kaggle community-originated} 
method to determine whether train and test datasets 
are drawn from the same distribution~\cite{ellis_2021}. 
Adversarial validation trains a binary classifier, 
$F(d)$, to predict whether a tuple $d$ came 
from either the train or test dataset. 
If $F(d)$ converges to $\sim$ 50\% AUC~\cite{ling2003auc}, 
then one can assume the datasets are 
similar~\cite{Pan2020AdversarialVA}. 
Extending this method to track 
shift seems straightforward: 
we can train $F(d)$ to predict whether $d$ 
comes from the training sample or 
the reservoir sample of prediction/live data 
(as in Section~\ref{sec:coarsegrained}), and log the AUC. 
However, adapting this method to the streaming 
setting is computationally challenging because 
we would need to train a new classifier $F(d)$ 
every time we log an AUC, 
and computing AUC requires multiple passes through the data.

\begin{figure}
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{figs/advc.pdf}
    \vspace{-15pt}
    \caption{AUC and log loss from the adversarial classifier over time, trained to separate a loss-weighted random sample of the training dataset and a reservoir sample of live tuples. The ML model accuracy is depicted by the dashed line.}
    \label{fig:advc}
    \vspace{-15pt}
\end{figure}

One insight is that users\techreport{ don't exactly care about the AUC,
they} only care about how the AUC changes over time, 
as an increasing AUC indicates that live data 
is diverging from training set data. 
As a proxy, we can log $F(d)$'s \emph{loss} over time, 
which can be computed in a single pass. 
To avoid frequently retraining $F(d)$ from scratch, 
every time we get a new tuple in the reservoir sample of live data, we can sample $d$ from the reservoir with $p=0.5$ and the training set with $p=0.5$; then, we can fine-tune $F(d)$ on $d$ with stochastic gradient descent. Here, the intuition is that decreases in loss are coupled with increases in AUC, as shown in Figure~\ref{fig:advc}. As loss decreases, it is becoming easier to separate the training and live data, indicating distribution shift. The onset of distribution shift as flagged by the adversarial classifier aligns with the beginning of the ML model accuracy drop (late March 2020).
The features highly weighted in $F(d)$ are also
the ones most likely to be responsible for the shift,
further aiding diagnosis.



% Most prior work in distribution shift for machine learning focuses on comparing two static datasets~\cite{failingloudly, wilds, mandoline, Ovadia2019CanYT}. However, in practice, we care about deploying models over infinite streams of data, or data for the foreseeable future. To approximately compute shifts in $P(X)$ and $P(Y)$, existing work proposes tracking metrics like KL divergence and the Kolmogorov-Smirnov tests between sliding windows in live inference data and train datasets (i.e., for train-serve skew as described in Breck et al. ~\cite{dataval}). These distance metrics need to be logged for all features ($P(X)$), predictions (estimates of $P(Y)$), and labels ($P(Y)$, when they come in). We can leverage the current reservoir or sample of live tuples (as described in Section~\ref{sec:coarsegrained}), but it is impractical to keep the entire training set in memory. We can keep a materialized sample of the training set in-memory, but randomly sampling the training set might neglect important tuples, such as those from minority classes. As a solution, we can obtain a weighted random sample of the train set, where each tuple is weighted by its loss.

% Tracking many distance metrics at scale isn't enough: this method suffers from $p$-values going to zero even if shifts aren't significant enough to warrant a retrain, as discussed in Section~\ref{sec:distshiftformal}. The ML community has explored adversarial validation as a means for determining whether two datasets $D$ and $D'$ are similar: if a binary classifier $F(d)$ trained to predict whether a tuple $d$ came from $D$ or $D'$ converges only to 50\% AuROC, then one can assume the datasets are similar enough~\cite{Pan2020AdversarialVA}. We can extend adversarial validation shift techniques to approximate distribution shift: we can periodically train $F(d)$ to predict whether $d$ comes from the training set sample or the reservoir sample of live data (as described in Section~\ref{sec:coarsegrained}), and log the AuROC. Adapting this procedure to the streaming setting is challenging because we would need to train a new classifier every time we want to log an AuROC. One insight is that users don't exactly care about the AuROC --- users care about knowing how the AuROC changes over time. As a proxy, we can instead fine-tune $F(d)$ over time, half on tuples from the training sample and half on new tuples in the live reservoir sample, and log $F(d)$'s \emph{loss} over time. The intuition here is that as loss decreases, it is becoming easier to separate the training and live data, indicating distribution shift.

% We can extend incremental metric computation~\cite{schelter} to support addition and removal of data points in the window of live inference data. 




==> integration.tex <==
\begin{Verbatim}[commandchars=\\\{\},numbers=left,firstnumber=1,stepnumber=1]
\colorbox{white}{\parbox{\linewidth}{\PY{k+kn}{import} \PY{n+nn}{pandas} \PY{k}{as} \PY{n+nn}{pd}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{\PY{k+kn}{from} \PY{n+nn}{sklearn}\PY{n+nn}{.}\PY{n+nn}{preprocessing} \PY{k+kn}{import} \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{n}{StandardScaler}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{\vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{\PY{n}{c} \PY{o}{=} \PY{n}{PreprocessingComponent}\PY{p}{(}\vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{    \PY{n}{name} \PY{o}{=} \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{preprocessing}\PY{l+s+s2}{\PYZdq{}}\PY{p}{,}\vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{    \PY{n}{owner} \PY{o}{=} \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{user}\PY{l+s+s2}{\PYZdq{}}\PY{p}{,}\vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{    \PY{n}{description} \PY{o}{=} \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{scaling}\PY{l+s+s2}{\PYZdq{}}\vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{\PY{p}{)}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{\vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{\PY{n+nd}{@c}\PY{o}{.}\PY{n}{run}\PY{p}{(}\PY{n}{input\PYZus{}vars} \PY{o}{=} \PY{p}{[}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{df}\PY{l+s+s2}{\PYZdq{}}\PY{p}{,} \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{features}\PY{l+s+s2}{\PYZdq{}}\PY{p}{]}\PY{p}{,}\vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{    \PY{n}{output\PYZus{}vars} \PY{o}{=} \PY{p}{[}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{train\PYZus{}df}\PY{l+s+s2}{\PYZdq{}}\PY{p}{,} \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{test\PYZus{}df}\PY{l+s+s2}{\PYZdq{}}\PY{p}{,} \vphantom{fg}}}
\colorbox{PaleGreen}{\parbox{\linewidth}{    \PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{s}\PY{l+s+s2}{\PYZdq{}}\PY{p}{]}\PY{p}{)}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{\PY{k}{def} \PY{n+nf}{preprocess\PYZus{}data}\PY{p}{(}\PY{n}{df}\PY{p}{,} \PY{n}{features}\PY{p}{)}\PY{p}{:}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{c+c1}{\PYZsh{} Splits df and standardizes}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{n}{train\PYZus{}df}\PY{p}{,} \PY{n}{test\PYZus{}df} \PY{o}{=} \PY{n}{rand\PYZus{}split}\PY{p}{(}\PY{n}{df}\PY{p}{)}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{n}{s} \PY{o}{=} \PY{n}{StandardScaler}\PY{p}{(}\PY{p}{)} \PYZbs{}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{o}{.}\PY{n}{fit}\PY{p}{(}\PY{n}{train\PYZus{}df}\PY{p}{[}\PY{n}{features}\PY{p}{]}\PY{p}{)}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{n}{train\PYZus{}df}\PY{p}{[}\PY{n}{features}\PY{p}{]} \PY{o}{=} \PYZbs{}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{n}{s}\PY{o}{.}\PY{n}{transform}\PY{p}{(}\PY{n}{train\PYZus{}df}\PY{p}{[}\PY{n}{features}\PY{p}{]}\PY{p}{)}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{n}{test\PYZus{}df}\PY{p}{[}\PY{n}{features}\PY{p}{]} \PY{o}{=} \PYZbs{}\vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{        \PY{n}{s}\PY{o}{.}\PY{n}{transform}\PY{p}{(}\PY{n}{test\PYZus{}df}\PY{p}{[}\PY{n}{features}\PY{p}{]}\PY{p}{)}   \vphantom{fg}}}
\colorbox{white}{\parbox{\linewidth}{    \PY{n}{save}\PY{p}{(}\PY{n}{train\PYZus{}df}\PY{p}{,} \PY{n}{test\PYZus{}df}\PY{p}{,} \PY{n}{s}\PY{p}{)}\vphantom{fg}}}
\end{Verbatim}

==> old_intro.tex <==
%!TEX root = main.tex

Organizations, big and small, are devoting increasingly more resources
towards developing and deploying applications powered by machine learning (ML). ML applications consist of pipelines that span multiple heterogeneous stages or \emph{components}, such as ETL and model training. These components each come with their own challenges, 
such as data preprocessing issues~\cite{schelter,dde,dagger}, 
dealing with covariate shift~\cite{sugiyama, dmc},
prediction serving problems~\cite{velox}, 
and periodic retraining complications~\cite{prodml}. 
As a result, practitioners assemble a myriad of tools
that each solve a fraction of challenges in a single component
with varying degrees of effectiveness.
For example, practitioners may use a Hive metastore to catalog frequently-changing raw data~\cite{hive}, Deequ for data validation~\cite{deequ}, and Weights \& Biases for experiment tracking during training~\cite{wandb}.

However, such a hodgepodge of tools threatens 
ML application \emph{sustainability}, 
or the ability to exist and 
continuously operate in production~\cite{mlsustainability}.
{\em The fundamental challenge underlying ML application sustainability
is the lack of end-to-end visibility into the ML pipeline.}
ML bugs could lie in any component in the end-to-end pipeline,
as well as in interactions between them~\cite{dmc}; moreover,
these pipelines could be complex even for a simple prediction task 
with only one model (Figure~\ref{fig:tradpipeline}). 
Furthermore, the pipeline doesn't stop existing once
a model is deployed---it continues to evolve
as models for the same task 
are periodically retrained and redeployed over time~\cite{prodml}.
To support visibility into specific components of the ML pipeline,
the database 
community has proposed a variety of solutions,
e.g., for identifying data bugs during 
preprocessing~\cite{mlinspect, dagger},
and for logging models and model metadata during training 
for post-hoc debugging~\cite{modeldb, mistique,modelhub,garcia2020hindsight}.
Additionally, industry solutions such as 
MLFlow~\cite{mlflow} and Weights \& Biases~\cite{wandb} 
have garnered widespread adoption by handling 
data management issues that stem from experimenting with large numbers of models.
Unfortunately, these piecemeal approaches do not address
the problem of \emph{cross-component} or end-to-end visibility into production ML pipelines,
thereby making debugging and maintenance difficult.

One promising approach for end-to-end visibility, 
and therefore ML application sustainability,
is to employ a holistic ML framework,
such as TFX~\cite{tfx} or Overton~\cite{overton}.
Users need to use the framework to implement all components---from 
data preprocessing to deployment---to benefit from it.
This rewrite can be cumbersome to users, who often prefer
to reuse their existing ML application code and avoid 
vendor lock-in~\cite{sagemaker, cloudy}.
Other approaches involve the use
of various best practices and understanding of 
failure case studies \cite{rubric, mldebt};
neither of which provide easy-to-use software solutions.
Instead, in this work, we propose a {\em lightweight, platform-agnostic 
system for supporting end-to-end ML application sustainability}.
To motivate the desired characteristics of such a system,
as well as the underlying challenges, we look to the concept 
of software {\em observability}~\cite{sridharan2018distributed}, and adapt it to the ML domain.

% Software companies are increasingly devoting more resources towards developing machine learning (ML) applications. These applications pose additional challenges to the software engineering lifecycle in data processing \cite{schelter,dde,dagger}, covariate shift \cite{sugiyama, dmc}, model training \cite{mlinspect}, and prediction serving \cite{velox}. To address these issues, practitioners pipe together a myriad of solutions that each solve individual problems in ML application development with varying degrees of effectiveness. A hodgepodge of tools can be challenging to maintain and threaten ML application \emph{sustainability}, or the ability to exist and continuously operate in production \cite{mlsustainability}.

% The DBMS community has embraced the challenges of supporting specific parts of ML pipelines, such as data preprocessing \cite{mlinspect, dagger} and model training \cite{mlflow, modeldb, mistique}. For instance, in model training, tools such as MLFlow \cite{mlflow} and Weights \& Biases \cite{wandb} have garnered widespread adoption because they effectively handle data management issues that stem from experimenting with large numbers of models. However, ML applications are difficult to maintain because bugs could lie anywhere in the end-to-end pipeline, which could be complex even for a simple prediction task with only one model (Figure \ref{fig:tradpipeline}). 

% The end-to-end space for ML is largely unexplored, with much of the end-to-end workflow support focusing on data analysis \cite{northstar, provdb}. "Production readiness" for ML applications has been been explored through lists of good practices and failure case studies \cite{rubric, mldebt}, but the field lacks research in building systems that enable such production-grade ML applications. The few tools that do support end-to-end production ML pipelines, including TFX \cite{tfx} and Overton \cite{overton}, force pipeline rewrites and vendor lock-in, thus requiring significant buy-in from users \cite{sagemaker, cloudy}. It can be impractical from a business perspective to migrate all ML application code, motivating a lightweight, platform-agnostic end-to-end ML application sustainability solution.

\begin{full}
To illustrate how ML applications can be difficult to maintain, suppose an end user reports some faulty predictions. First, models almost always have some error, so it is unclear if these predictions are unexpected mistakes. Second, if we conjecture that the pipeline has a bug, it is unclear where the bug might be. Is the model stale? Are the features incomplete? Is the raw data corrupted in some way? Third, from an end-to-end view, ML pipelines can be incredibly complex and consist of many data transformations and ML models, making it unlikely for a single rotating on-call engineer or data scientist to easily triage an issue.

ML observability could be simpler to implement when each component of the end-to-end pipeline is developed and executed in the same framework \cite{tfx, overton, sagemaker, cloudy}. However, many organizations employ multiple tools and frameworks in their pipelines \shreya{include figure with how complicated the ml stack can get, maybe compared to the software stack}, and it can impractical from a business perspective to migrate all existing data collection, processing, and software endpoint serving components to a single framework. Achieving ML observability for such organizations can require large, dedicated ML infrastructure teams \cite{michelangelo}, motivating a flexible, platform-agnostic tool.
\end{full}

\subsection{ML Observability}

\begin{full}
The ability to ask questions about bugs in system behavior is a precursor to having a long-lasting production-grade system. Examples of questions that ML practitioners may want to ask are:

\begin{itemize}
    \item Why did my users complain about my recent predictions?
    \item When should I retrain my model?
    \item What steps were involved in producing this output?
    \item Can I delete this folder of models without breaking production?
\end{itemize}

Like software observability tools, ML observability tools could capture "snapshots" of the system in the form of logs, metrics, and traces, which must be synthesized and presented to the developer.

\topic{Logs} Three main challenges stem from logging for ML pipelines: (1) constructing a common schema for data and metadata to log during each stage, (2) using little space to store the information, and (3) having minimal pipeline runtime overhead. Several existing works focus on logging at specific stages such as cluster deployment, preprocessing, training, and serving \cite{mlflow, modeldb, provdb, lima}. Even if an organization uses such tools, many ML pipelines consist of stages that are developed by different people, so it can be hard for a single person to find and understand the logs from each stage. Additionally, the patterns and needs of logging at different stages are different -- for example, a training stage could require a hyperparameter search, which could yield thousands of new models, but an inference stage that supports "online" learning may only yield one model -- making it tedious to "chain" logs together to support end-to-end logging. 

\topic{Metrics} In software, metrics are defined as numerical values that capture system health over a time interval. Traditionally, this includes average response time or median number of crashes. Machine learning pipelines require additional metrics that shed insight into model performance, which could be challenging to measure in a production inference setting where there are no immediate labels given as feedback. Furthermore, estimating distribution shift based only on observed data points and limited sample sizes could be difficult \cite{dataval}. The number of metrics can scale with input and output dimensionalities, making it hard to present these metrics to the user in a readable way. 

% Existing work highlights monitoring simple reductions over inputs and outputs such as the mean and median and captures a notion of train-inference skew with well-known distance metrics such as KL divergence \cite{tfx, dataval}. TFX has a custom distance metric based on Dirichlet priors, but this method requires the distributions to contain at least 1 billion points and the $n$ observed samples to be independently and randomly drawn, not the last $n$ data points observed by the model in production. In Google's case, the method may work because the sheer number of predictions made can be high enough to meet the 1 billion threshold in a relatively short amount of time. The method may not work at a smaller company where the data volume is not so high. 

\topic{Traces} Traces, which represent the end-to-end journey for data, can help identify where the pipeline broke down if there was a bug. In software, the unit of data is typically a request, where the trace tracks all the steps involved in creating the response delivered. ML pipelines similarly require tracing for any output, but additional challenges arise because there can be silent failures, each stage can have many inputs and outputs, and the inputs and outputs of these stages may not be versioned. Much related work focuses on data and model versioning \cite{versiontradeoff, orpheus}, provenance tracking, data and ML code inspection tools \cite{mlinspect, slicefinder, vizier}, and workflow management \cite{mlflow, modelhub, provdb}, at different stages of the pipeline. However, to get true observability, tracing must be done across all stages of the pipeline in an end-to-end fashion. Finer-grained tracing can be hard when each stage relies on a different language and/or tool.

An ideal solution integrates logging, measuring metrics, and tracing to allow any engineer or data scientist involved in building an ML application to ask a variety of questions about an ML pipeline's health. This is particularly challenging to do for ML pipelines because engineers and data scientists do not have largely overlapping skill sets -- engineers know \emph{how} to log, measure, and trace; data scientists know \emph{what} to log, measure, and trace. Observability requires a strong intuition for both.
\end{full}

\begin{figure*}
\vspace{-15pt}
    \centering
    % \begin{subfigure}[c]{0.49\linewidth}
    % \includegraphics[width=\textwidth]{tradpipeline.eps}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[c]{0.49\linewidth}
    % \includegraphics[width=\textwidth]{architecture.eps}
    % \end{subfigure}
    \includegraphics[width=0.8\textwidth]{tradpipeline.pdf}
    % \vspace{-5pt}
    \caption{High-level architecture of a generic end-to-end machine learning pipeline. Logos represent a sample of tools used to construct components of the pipeline, illustrating heterogeneity in the tool stack.}
    \label{fig:tradpipeline}
% \vspace{-10pt}
\end{figure*}


Software observability~\cite{sridharan2018distributed} is a concept drawn from control theory,
and refers to bringing  ``{\em better visibility into understanding the complex
behavior of software using telemetry collected ... at run time''}~\cite{karumuri2021towards}. 
Existing software observability tools 
lack support for ML pipelines, 
which require many additional performance metrics 
and frequent "snapshotting" due to ever-changing 
data flow through the pipeline, 
posing new research challenges in data management. 

Typical software observability solutions 
present metadata in the form of \emph{logs}, \emph{metrics}, 
and \emph{traces}\techreport{\footnote{\scriptsize{\em Events} is another form of software observability artifact; however
they are less relevant in an ML setting~\cite{karumuri2021towards}. These artifacts are together referred to as MELT.}} 
and synthesize this information to 
allow engineers to ask questions about system health.
ML applications add new criteria to system health, 
as performance extends beyond system uptime; 
it also relies on the quality of predictions 
or outputs. 
We use the three aforementioned pillars of software observability 
as inspiration for the key facets of our ML observability approach, and outline the corresponding research challenges, next\footnote{\scriptsize Logs, metrics, and traces,
as used in software observability, represent different debugging patterns (i.e., finding a "needle in a haystack," inspecting the cause of an alert, and understanding the lifecycle of an action respectively). 
These debugging patterns and corresponding metadata 
do not map directly
to ML observability, motivating our slight modification.}.

\topic{Logging} 
Traditional software applications record events
through logs, or event-related metadata produced
at runtime, such as stack traces and error codes.
While debugging, users search these logs post-hoc
to answer their "needle-in-a-haystack" queries.
ML applications add complexity to logging
since they can experience silent failures 
(e.g., covariate shift or concept drift),
which may not be reflected in typical output or error logging statements.
Thus, our approach must capture inputs and outputs
of intermediate components, both of which can be computationally
expensive and bulky to store (e.g., large DNN models).
Additionally, it must be able to identify how inputs and outputs
feed into each other across the pipeline, despite pipeline
components being run at various frequencies, e.g.,
the ETL step in Figure~\ref{fig:tradpipeline} being run weeks prior to Inference.
It should also support this logging in a lightweight manner
with minimal user input.

%ML adds complexity to logging because ML pipelines can experience silent failures (i.e. covariate shift), most of which may not even show up in STDOUT, let alone STDERR. Our observability solution would need to log extra information, such as statistics of inputs and outputs, which can be both computationally expensive and bulky to store.

\topic{Monitoring} 
In traditional software applications, 
engineers monitor numerical metrics 
that directly represent how well 
an application is performing (i.e., mean response time) 
and receive alerts when these metric values exceed 
a predefined threshold. 
Such metrics are typically simple 
to measure, as the values can easily be 
captured in the application and 
aggregations are straightforward. 
Monitoring is not straightforward in ML
because the success of an ML application 
depends on model performance, 
which cannot easily be measured;
labels, or true values, are often 
not provided in real-time in the production endpoint. 
Even if direct feedback 
is available (e.g., when a user clicks on an ad), 
ML metrics, such as F1 and t-test scores, 
can be expensive to compute at scale.
Our approach must support a variety of ML-centric
metrics efficiently in a plug-and-play fashion 
without the user having to write a lot of code,
with these metrics being tracked in-situ as components
of the pipelines are run repeatedly. 
Users should also be able to set alerts, triggers,
or constraints to ensure overall ML pipeline health. 


\topic{Querying} 
To debug systems from a holistic, end-to-end perspective, 
users need to be able to query the logs and metrics produced by an observability tool. To debug traditional software applications, engineers typically first inspect a trace, 
or the end-to-end journey of a data point, 
to understand the lineage of that request 
and determine where the bug may lie. 
This lineage may be straightforward to track 
when transformations are done in a single framework (e.g., REST), 
but ML applications are built 
using heterogeneous stacks of many tools. Having a complicated technical stack fragments access to information about data flow and provenance. 
Our approach must therefore integrate 
with a heterogeneous set of 
tools and still support lineage tracking.
Second, ML bugs are rarely constrained to a single output, as ML pipelines will not have 100\% accuracy. Practitioners typically investigate errors belonging to a group of outputs, or a \emph{slice}.
Our approach must support slice-based lineage querying where slices could be any subgroup defined on-demand, efficiently. Third, in many regulated industries such as finance or law, users may need to query over previous months or even years, requiring data to be retained over unusually long periods of time. This differs from traditional software applications, which commonly retain metadata on the order of days or weeks.


% We frame "production ML" challenges through the lens of \emph{observability}, or visibility into the end-to-end performance of an application. Existing software observability tools lack support for ML pipelines, which require many additional performance metrics and ultra-frequent "snapshotting" due to ever-changing data flow through the pipeline, posing new research challenges in data management. 

% In order to plug an ML observability solution into the software engineering ecosystem, key facets of the solution must mirror how software observability solutions are designed. Software observability solutions capture data in the form of \emph{logs}, \emph{metrics}, and \emph{traces} and synthesize this information to allow engineers to ask questions about system health. ML applications add new criteria to system health, as ML application performance extends beyond system uptime; it also relies on the quality of predictions or outputs.
\begin{full}
\topic{Logs} Although code may not change, data is constantly changing, requiring information such as inputs and outputs to be logged any time any stage of a pipeline is run. Thousands of outputs could be generated daily even in small organizations, and if users want to query across months of runs, it could be challenging to return results quickly, let alone store all of these logs.

\topic{Metrics} While logs are artifacts, metrics are aggregations of artifacts over arbitrary, user-defined periods of time. These aggregations, such as KL divergence, could be costly to compute at scale across high-dimensional data. Additionally, users may not know what metrics are most relevant to their pipeline health, as different prediction tasks follow different data distributions and thus require different metrics. Our tool would need to suggest metrics for users to measure.

\topic{Traces} The end-to-end journey of a data point may be straightforward to track when transformations are done in a single framework, but ML applications are built using heterogeneous stacks of many tools. Having a complicated technical stack fragments access to information about data flow and provenance. Additionally, traces, or post-hoc queries on computation graphs, need to be computed quickly for a good user experience.
\end{full}


\subsection{\Large \mltrace}
In this paper, we discuss research challenges in building a "bolt-on" observability system for ML pipelines, or a solution that does not require users to rewrite all their code to use a specific framework, as as a call-to-arms for the database community
to contribute to this nascent research
direction. We propose an example of a bolt-on ML observability system called \mltrace, which has
already received preliminary interest
from practitioners with over 300 GitHub stars (\texttt{github.com/loglabs/mltrace}). \mltrace is a lightweight end-to-end
 framework
centered around the execution of individual pipeline components that will eventually support: 
({\em i}) automatic logging of component
run metadata, inputs, and outputs, ({\em ii}) a pluggable library
of metrics and alerts to sustain ML performance ({\em iii}) a flexible querying framework and UI for users to debug their pipelines.
\mltrace flexibly interoperates with existing tools used in ML 
application development,
and provides logging, monitoring, and querying capabilities
to data scientists and engineers who like fine-grained control
across the end-to-end pipeline.


% We address the ML observability problem with \mltrace{}, a lightweight, end-to-end framework centered around the execution of individual components in a pipeline. Our vision is to offer flexible logging, testing, and monitoring to data scientists and engineers that like to have fine-grained control over their pipelines. We have designed for it to be used in conjunction with other tools that help develop specific components of the pipeline. In this paper, we lay out the architecture for \mltrace{}, demonstrate the current prototype, and describe further research challenges in working towards our vision for \mltrace{}. 

% Just like software pipelines, ML pipelines inevitably have bugs in production, no matter how many sanity checks exist. Performing a rollback to an earlier snapshot of the pipeline can aid in debugging. This is easy to do in traditional software applications; a user could check out the relevant version of the codebase with one command. Unfortunately, rollbacks are more complicated in ML applications, where code is not the only first-class citizen anymore. Data, models, and artifacts may be housed, versioned, and managed differently. Lack of observability forces organizations does not need to build a rollback tool for themselves.

\begin{full}
Large companies that work on ML tooling have lots of incentives to "lock" their customers into their developer ecosystems, making it unlikely for them to work on platform-agnostic ML observability tools. Much of the academic community's work in ML lifecycle management focuses on either a particular stage in the lifecycle or the lifecycle up to serving the model \cite{mlflow, modeldb, dagger, lima, mlinspect, keystone}. While these solutions give great insight into certain parts of developing ML applications, observability after an ML pipeline has a production release is largely unexplored in an academic context. We posit there are many interesting problems in this domain for the DBMS community.

In this paper, we discuss characteristics of ML pipelines, propose criteria for ideal ML pipeline observability, describe relevant challenges in working towards such a vision, and introduce \mltrace{}, our open source platform-agnostic tool to instrument ML pipelines to achieve observability. We propose a flexible logging schema and describe data flow tracking mechanisms in \mltrace{} that can enable end-to-end logging, tracing, and monitoring. We showcase the current prototype and discuss its roadmap. 
\end{full}


% \begin{itemize}
%     \item Blah blah everyone is doing ML in software
%     \item Lots of things are going wrong in developing these pipelines
%     \begin{itemize}
%         \item ML software dev is much more data-centric
%         \item Lots of artifacts
%         \item Lots of stages (ingest, ETL, train, val, retrain, inference, etc)
%     \end{itemize}
%     \item Developers, especially teams of developers, just do not know what their ML software's failure modes are
%     \item A whole field of MLOps has emerged in industry to try an address these issues. Many researchers have also devoted attention. Space is crowded
%     \item We posit that the software concept of observability is extremely relevant in this data-centric paradigm of software engineering, and doesn't really exist
%     \item Our contributions:
%     \begin{itemize}
%         \item Discussion of observability
%         \begin{itemize}
%             \item the separation of DevOps and software engineers, Agile methodologies to facilitate collaboration
%             \item similar trend in separating data scientists and data / ML engineers, but the collaboration processes are nearly nonexistent. Agile is hard when data scientists are not trained engineers (they don't need to be), DS workflows are not repoducible and produce hella artifacts (ex: hparam sweep a bunch of different ideas just to make one model binary to deploy to prod)
%             \item There's a number of tools to aid in developing specific components of the pipeline, but there is no tool to answer "how are your production ML applications performing right now?"
%         \end{itemize}
%         \item Framing the problems in end-to-end data \& ML application development in the lens of observability (metrics, logs, and tracing to identify \emph{when} and \emph{why} things go wrong)
%         \item Discussion on the challenges of having good observability in data-intensive systems
%         \item \emph{mltrace}, an open source platform agnostic tool to instrument ML codebases to achieve observability
%         \item A vision for seamless collaboration on ML applications, enabling data scientists and engineers to work towards optimizing for the same metrics
%     \end{itemize}
% \end{itemize}

==> pipeline.tex <==
\begin{figure*}[!t]
\vspace{-10pt}
    \centering
    \includegraphics[width=0.8\linewidth]{architecture.pdf}
\vspace{-5pt}
    \caption{Proposed \mltrace{} architecture}
    \label{fig:architecture}
% \vspace{-15pt}
\end{figure*}

We now explain common properties of production ML pipelines and unaddressed observability-related needs.
The beginning of an end-to-end ML pipeline corresponds to data collected directly from the most upstream source imaginable, with the end being the most downstream output given to a user. For example, suppose a ride-sharing company has an ML application that tells drivers how likely their user is to give a tip. One end of this pipeline would be the mobile app telemetry data, and the other end would be the predicted tip probability shown to the driver. Although the task could be simple, such pipelines, can be complex and consist of many components. The notion of a component is flexible: for example, each box in the ML pipeline shown in Figure~\ref{fig:tradpipeline} can be a component.


\subsection{Properties of Pipelines}

\topic{Pipeline architecture is dynamic} Rarely is the architecture for an ML pipeline known upfront. As ML pipelines stand in production over time, new components are added and existing components are removed. For instance, a data scientist may add a new model to a pipeline to boost performance via ensembling, which could add new preprocessing, training, and inference components. Thus, \emph{logging must be done at the component level}, not the pipeline level.

\topic{Components are dynamic} Not only do pipelines change, but a single component itself can easily change. In the software world, components change when code changes. Every pull request to a production codebase triggers a suite of continuous integration (CI) tests, written outside the main application in a \texttt{tests} folder, to verify functionality. In the ML world, components can also change when any data or artifact (e.g., saved function or model) changes, rendering the software mechanism of CI testing insufficient. Thus, \emph{our solution must execute tests on inputs and outputs at component runtime.} Tools like Deequ~\cite{deequ} and TFX~\cite{tfx} allow users to write data quality tests to execute at component runtime; however such tests are written as part of the main application and therefore not easily reusable. 

\begin{full}
\subsection{Components DEPRECATED}
\aditya{fix flow into this subsection, maybe say something
about various characteristics of the components}
\topic{Interactions between components} Components in the same pipeline change at different frequencies. 
For example, a data engineer may fix a SQL bug in an ETL
component while the inference component stays the same. \aditya{This doesn't illustrate different frequencies}
This indicates that logging should be performed at the component level, not the pipeline level.

\topic{Dynamic pipelines} Rarely is the architecture for an ML pipeline fixed and known at the time it is first constructed. As ML pipelines stand in production over time, new components can be added and existing components can be removed. For instance, a data scientist may add a new model to a pipeline to boost performance via ensembling, which could add new preprocessing, training, and inference components.

\topic{Dynamic components} Not only do pipelines change, but a single component itself can easily change. In the software world, components change when code changes. Every pull request to a production codebase triggers a suite of continuous integration (CI) tests, written outside the main application in a \texttt{tests} folder, to verify functionality. In the ML world, components can also change when any data or artifact changes, rendering the software mechanism of CI testing insufficient. Organizations adopt useful tools like Deequ~\cite{deequ} and TFX~\cite{tfx} to write data quality tests to execute at component-level runtime; however such tests are written as part of the main application and thus not reusable across applications.
\end{full}


\subsection{User Needs}
\label{sec:userprobs}


\begin{full}
Like other constantly changing systems, ML pipelines can have numerous problems, making them tedious to maintain. ML applications suffer from silent failures, or bugs that neither trigger any reporting nor halt computation. The potential for bugs in the end-to-end system is limitless: a broken sensor could report \texttt{NaN}s in a data ingestion component, an ETL component could have an off-by-one error on SQL windowing, a training component could have train-test leakage, and more. It is unrealistic to expect a single system to address every bug in class of ML pipeline problems. The goal for our observability system is for the user to be able to ask \emph{how} the end-to-end system is behaving and specify their own "triggers" and "constraints" in their pipeline to safeguard against future bugs.
\aditya{and present ones? it may not be clear to
readers why a trigger or a constraint would be valuable
in this context.} 
\end{full}

To debug their pipelines, practitioners need to query across different \emph{states} of components. We define component state to represent information recorded or updated at component runtime, such as inputs, outputs, code snippets, start time, git hash, and other component metadata. We categorize common ML observability questions into four categories of increasing complexity:

\begin{enumerate}
    \item \textbf{Component run-level queries} include questions about a specific run of a component, such as specific input values or fine-grained component execution failures.
    \item \textbf{Component history queries} include questions about historical behavior of a component, such as whether there is data drift.
    \item \textbf{Cross-component queries} include questions about how components interact with each other, such as whether there is a mismatch between the online and offline sub-pipelines.
    \item \textbf{Cross-component history queries} include questions about historical pipeline snapshots, such as traces for a slice of outputs.
\end{enumerate}

% \vspace{1pt}

% \noindent \textbf{1. Component run-level queries} include questions about a specific run of a component, such as specific input values or fine-grained component execution failures.
% \vspace{1pt}

% \noindent \textbf{2. Component history queries} include questions about historical behavior of a component, such as whether there is data drift.
% \vspace{1pt}

% \noindent \textbf{3. Cross-component queries} include questions about how components interact with each other, such as whether there is a mismatch between the online and offline sub-pipelines. 
% \vspace{1pt}

% \noindent \textbf{4. Cross-component history queries} include questions about historical pipeline snapshots, such as traces for a slice of outputs.
% \vspace{0.5pt}

To address these queries, an ML observability system must be able to compute and store (1) history of and (2) interactions between components, motivating our key design decision to log state and perform user-defined "triggers" at component runtime. The system can then reconstruct the pipeline computation DAG to help practitioners catch failures.

% To achieve ML application observability, not only do we need to log information every time a component is run, but the user will need to interact with this information to answer questions they may have about the pipeline.

==> roadmap.tex <==
\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\small
% \setlength\tabcolsep{3pt}
  \begin{flushleft}
    \begin{tabularx}{0.95\linewidth}{>{\raggedleft}p{0.18\linewidth}>{\raggedright}p{0.18\linewidth}|>{\raggedright}p{0.21\linewidth}|>{\raggedright\arraybackslash}p{0.21\linewidth}}
    %   \toprule % <-- Toprule here
    %   \textbf{Detect} & \textbf{Diagnose} & \textbf{React}\\
    %   1 & 2 & 3 \\
    \multicolumn{1}{c}{}&\multicolumn{1}{c}{\framebox(0.7in, 0.2in){\textbf{Detect}}\tikzmark{aa}}&\multicolumn{1}{c}{\tikzmark{bb}\framebox(0.7in, 0.2in){\textbf{Diagnose}}\tikzmark{cc}}&\multicolumn{1}{c}{\tikzmark{dd}\framebox(0.7in, 0.2in){\textbf{React}}}\\
    %   \midrule % <-- Midrule here
    %   \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &\multicolumn{1}{c}{}  & \multicolumn{1}{c}{} \\
    %\textbf{Question} & {\em What is performance like?} & {\em What are components at a given time} & {\em  \\
    \textbf{Objective} & Track {\em holistic} ML metrics (e.g., accuracy) & Identify {\em point-in-time component-level} issues & Assist fixing {\em cross-component, cross-time} issues\\
    % \midrule
    \multirow{2}{*}{\textbf{Challenges}} & Missing labels (\Cref{sec:nofeedback}) & Precise data quality constraints (\Cref{sec:dataconstraints}) & Unexpected feedback delays  (\Cref{sec:react-label}) \\
    & Delayed labels (\Cref{sec:partialfeedback}) & Natural data drift  (\Cref{sec:distshift}) & Pipeline-wide errors  (\Cref{sec:react-component}) \\
    %  \bottomrule 
    \end{tabularx}
    \begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, shorten <=.5pt, transform canvas={yshift=.65\baselineskip}]
        \draw [->] ({pic cs:aa}) -- ({pic cs:bb});
        \draw [->] ({pic cs:cc}) -- ({pic cs:dd});
    \end{tikzpicture}
  \end{flushleft}
\end{table}
